MobileForge: Annotation-Free Adaptation for Mobile GUI Agents with Hierarchical Feedback-Guided Policy Optimization

MLLM-based mobile GUI agents have made substantial progress in UI understanding and action execution, but adapting them to real target apps remains costly because mobile apps are numerous, frequently updated, and hard to cover with human-written tasks, demonstrations, or reward labels. Existing annotation-free GUI learning reduces manual supervision, yet lacks a unified substrate connecting target-app exploration, curriculum mining, rollout execution, and feedback, while policy optimization often relies on isolated rollouts and coarse rewards that are hard to convert into reliable improvement signals. We present MobileForge, an annotation-free adaptation system for mobile GUI agents. MobileForge consists of MobileGym, which grounds task generation and rollout evaluation in real mobile app interaction, and Hierarchical Feedback-Guided Policy Optimization (HiFPO), which turns trajectory outcomes, step-level process feedback, and corrective hints into hint-contextualized step-level GRPO updates. Using only automatically generated annotation-free adaptation data, MobileForge adapts Qwen3-VL-8B to 67.2% Pass@3 on AndroidWorld, close to the closed-data GUI-specialized GUI-Owl-1.5-8B base model at 69.0%. The MobileForge-adapted ForgeOwl-8B further reaches 77.6% Pass@3 on AndroidWorld and 41.0% success on the out-of-domain MobileWorld GUI-only split, establishing the strongest open-data mobile GUI agent in our evaluation. Code, data, and trained models will be released at https://mobile-forge.github.io/.

==> tables/table-related-work-comparison.tex <==
\begin{table*}[t]
\centering
\paperCompactTable
\caption{Comparison with annotation-free GUI agent learning and adaptation methods. We organize the comparison around two limitations addressed by \ourmethod: the lack of a unified mobile interaction and evaluation substrate, and the reliance on isolated rollout experience with coarse or sparse feedback.}
\label{tab:related_work_comparison}
\begin{paperFit}[\textwidth]
\begin{tabular}{l l c c c l c l}
\toprule
\textbf{Method} &
\textbf{Main Source / Setting} &
\multicolumn{3}{c}{\textbf{Pain Point 1: Mobile Interaction and Evaluation Substrate}} &
\multicolumn{3}{c}{\textbf{Pain Point 2: Feedback-to-Optimization}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
&
&
\makecell{\textbf{Target Mobile}\\\textbf{Interaction}} &
\makecell{\textbf{Auto Task /}\\\textbf{Curriculum}} &
\makecell{\textbf{Hierarchical}\\\textbf{Rollout Eval.}} &
\makecell{\textbf{Feedback}\\\textbf{Granularity}} &
\makecell{\textbf{Cross-Attempt}\\\textbf{Experience}} &
\makecell{\textbf{Policy}\\\textbf{Update}} \\
\midrule
TongUI & Web tutorials & \pmark & \xmark & \xmark & Tutorial-derived trajectories & \xmark & SFT \\
MobileA3gent & User phone trajectories & \pmark & \xmark & \xmark & Auto-annotated instructions & \xmark & SFT / FL \\
GUI-explorer & Autonomous app exploration & \cmark & \pmark & \xmark & Transition-aware knowledge & \pmark & \xmark \\
OS-Genesis & Reverse task synthesis & \pmark & \cmark & \pmark & Trajectory reward model & \xmark & SFT \\
ZeroGUI & Online GUI rollout & \pmark & \cmark & \pmark & Trajectory-level VLM reward & \xmark & Online RL \\
MobileGUI-RL & Online mobile rollout & \cmark & \cmark & \pmark & Trajectory-level composite reward & \xmark & MobiGRPO \\
SEAgent & Desktop software & \xmark & \cmark & \pmark & Step-wise assessment & \pmark & GRPO + imitation \\
ACuRL & Computer-use environments & \xmark & \cmark & \pmark & Outcome evaluator / CUAJudge & \pmark & Curriculum RL \\
UI-Oceanus & Synthetic GUI dynamics & \pmark & \cmark & \xmark & Transition objectives & \xmark & CPT + SFT \\
\midrule
\rowcolor{oursrowcolor}
\textbf{\ourmethod} &
\textbf{Target mobile apps} &
\cmark &
\cmark &
\cmark &
\makecell[l]{\textbf{Trajectory outcome}\\\textbf{+ step-level process}\\\textbf{+ corrective hints}} &
\cmark &
\textbf{\hifpo} \\
\bottomrule
\end{tabular}
\end{paperFit}
\vspace{2pt}
\begin{flushleft}
\footnotesize
\cmark: explicitly supported; \pmark: partially supported or not specific to annotation-free mobile adaptation; \xmark: not supported or not the focus. \mobilegym covers the interaction and evaluation substrate, while \hifpo covers cross-attempt experience reuse and policy optimization.
\end{flushleft}
\end{table*}

